Multiscale deep context modeling for lossless point cloud geometry compression

We propose a practical deep generative approach for lossless point cloud geometry compression, called MSVoxelDNN, and show that it significantly reduces the rate compared to the MPEG G-PCC codec. Our previous work based on autoregressive models (VoxelDNN) has a fast training phase, however, inference is slow as the occupancy probabilities are predicted sequentially, voxel by voxel. In this work, we employ a multiscale architecture which models voxel occupancy in coarse-to-fine order. At each scale, MSVoxelDNN divides voxels into eight conditionally independent groups, thus requiring a single network evaluation per group instead of one per voxel. We evaluate the performance of MSVoxelDNN on a set of point clouds from Microsoft Voxelized Upper Bodies (MVUB) and MPEG, showing that the current method speeds up encoding/decoding times significantly compared to the previous VoxelDNN, while having average rate saving over G-PCC of 17.5%. The implementation is available at https://github.com/Weafre/MSVoxelDNN.

==> complexity.tex <==
We compare computational complexity of MSVoxelDNN and VoxelDNN using number of floating point operations (FLOPs) used by neural networks in encoding/decoding process. This number is highly affected by the complexity of network itself and also how many network evaluations are performed. For each network, we compute number of FLOPs on each layer and sum up to get the total FLOPs. For example, the number of FLOPs of a normal 3D convolution with kernel size $K$, $C_{in}$ the input chanels, $D_{out}, H_{out}, W_{out}$ the output dimensions and $C_{out}$ the output chanel is: 
\begin{equation}
    FL_{3DCNN}=K^{3}\times C_{in}\times (D_{out}\times H_{out}\times W_{out})\times C_{out}
\end{equation}
For a masked 3D convolution, we have additional operations for element wise multiplication between mask and filter: 
\begin{equation}
    FL_{Masked-3DCNN}= FL_{3DCNN} + K^{3}\times C_{in}\times C_{out}
\end{equation}
3D-ResNet skip connection requires a number of additions:
\begin{equation}
    FL_{Skip}= D_{out}\times H_{out}\times W_{out} \times C_{out}
\end{equation}
The other layers such as activation, split, merge are commonly not counted as they only take up a small fraction of the execution time. 
\par We report the number of network evaluations on a single block 64 of MSVoxelDNN and VoxelDNN for both encoder, decoder as well as the total FLOPs (worst case scenario) in Table \ref{table:complexityflops}. We observe that, VoxelDNN theoretically consumes significant more operations on both encoder and decoder side. On the encoder side, VoxelDNN performs 1 network evaluation per block in all resolutions with the number of blocks growing exponentially while MSVoxelDNN always has 8 network evaluations on higher scales and a single VoxelDNN of size 8 in the base scale. The number of FLOPs of VoxelDNN encoder is about 3 times of MSVoxelDNN. It explodes to  156655 times when VoxelDNN decoder must perform one network evaluation per voxel (worst case) while MSVoxelDNN can predict multiple voxels in parallel except the base layer with sequential predictions. Note that in practice, VoxelDNN partitions a block into sub-blocks in which some of them can be empty and thus, it can perform network evaluations on lower resolutions with much lower number of voxels. We only provide the number of FLOPs to have a general idea about computational complexity, this is not the exact measurement for running time of each methods.

\input{table-network-evaluation}

==> table-model-sizes.tex <==
\begin{table}[t]
\caption{Input, Output of all predictors for a $2D\times2D\times2D$ block. LR stands for Lower Resolution.}
\centering
\resizebox{0.97\linewidth}{!}{ \begin{tabular}{R{1.8cm}R{1.7cm}R{1.8cm}R{1.5cm}}
\hline


 \begin{bf}Input Group\end{bf} 
&\begin{bf}Input Size\end{bf}
& \begin{bf}Output Group\end{bf} 
& \begin{bf}Output Size\end{bf} \\
\hline

LR&$D\times D \times D$& 1& $D\times D \times D$\\
1&$D\times D \times D$& 2& $D\times D \times D$\\
1,2&$D\times D \times 2D$& 3& $D\times D \times D$\\
1,2,3&$D\times 2D \times 2D$& 4& $D\times D \times D$\\
1,2,..4&$D\times 2D \times 2D$& 5& $D\times D \times D$\\
1,2,..5&$2D\times 2D \times 2D$& 6& $D\times D \times D$\\
1,2,..6&$2D\times 2D \times 2D$& 7& $D\times D \times D$\\
1,2,..7&$2D\times 2D \times 2D$& 8& $D\times D \times D$\\


\hline
\end{tabular}}
\label{table:modelsize}
\end{table}

==> table-network-evaluation.tex <==
% \begin{table}[t]
% \caption{Complexity comparision between MSVoxelDNN and VoxelDNN for single block prediction (worse case scenario). $N \times V(D)$ stands for $N$ VoxelDNN of size $D$ evaluations. For MSVoxelDNN, $N \times M(D)$ is $N$ evaluations at scale $D$. }
% \centering
% \resizebox{0.97\linewidth}{!}{ \begin{tabular}{R{1.8cm}cR{1.8cm}}
% \hline


%  \begin{bf}VoxelDNN\end{bf} 
% & \begin{bf}Encoder\end{bf} 
% & \begin{bf}MSVoxelDNN\end{bf} \\
% \hline

% 1$\times $V(64)& &8$\times $M(64)\\
% 8$\times $V(32) &&8$\times $M(32) \\
% 64$\times $V(16)&&8$\times $M(16)\\
% 256$\times $V(8)&& 1$\times $V(8)\\
% \textit{266.5 B} & \textit{Total FLOPs }&\textit{89.4 B} \\


% & \begin{bf}Decoder\end{bf} 
% &  \\
% \hline

% \multirow{4}{*}{64$^3$$\times $V(64)}& &8$\times $M(64)\\
%  &&8$\times $M(32) \\
% &&8$\times $M(16)\\
% && 256$\times $V(8)\\
% \textit{19962809 B} & \textit{Total FLOPs}&\textit{127 B} \\

% \hline
% \end{tabular}}
% \label{table:complexityflops}
% \end{table}

\begin{table}[t]
\caption{Complexity comparision between MSVoxelDNN and VoxelDNN for single block prediction (worse case scenario). $N \times V(D)$ stands for $N$ VoxelDNN of size $D$ evaluations. For MSVoxelDNN, $N \times M(D)$ is $N$ evaluations at scale $D$. }
\centering
\resizebox{0.97\linewidth}{!}{
\begin{tabular}{R{1.8cm}cR{1.8cm}}
\toprule


 \begin{bf}VoxelDNN\end{bf} 
& 
& \begin{bf}MSVoxelDNN\end{bf} \\
\midrule
& \begin{bf}Encoder\end{bf} & \\

1$\times $V(64)& &8$\times $M(64)\\
8$\times $V(32) &&8$\times $M(32) \\
64$\times $V(16)&&8$\times $M(16)\\
256$\times $V(8)&& 1$\times $V(8)\\
\textit{266.5 B} & \textit{Total FLOPs }&\textit{89.4 B} \\

\midrule
& \begin{bf}Decoder\end{bf} &  \\
% \midrule

\multirow{4}{*}{64$^3$$\times $V(64)}& &8$\times $M(64)\\
 &&8$\times $M(32) \\
&&8$\times $M(16)\\
&& 256$\times $V(8)\\
\textit{19,962,809 B} & \textit{Total FLOPs}&\textit{127 B} \\

\bottomrule
\end{tabular}
}
\label{table:complexityflops}
\end{table}
